The Reactive Synthesis Competition: SYNTCOMP 2016 and Beyond

We report on the design of the third reactive synthesis competition (SYNTCOMP 2016), including a major extension of the competition to specifications in full linear temporal logic. We give a brief overview of the synthesis problem as considered in SYNTCOMP, and present the rules of the competition in 2016, as well as the ideas behind our design choices. Furthermore, we evaluate the recent changes to the competition based on the experiences with SYNTCOMP 2016. Finally, we give an outlook on further changes and extensions of the competition that are planned for the future.

==> eptcsdata.tex <==
\providecommand{\firstpage}{133}
\providecommand{\publicationstatus}{Dimitrova, Piskac (Eds.): Fifth Workshop on\\ 
Synthesis (SYNT 2016)\\
EPTCS 229, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.229.11}{10.4204/EPTCS.229.11}}
\usepackage{ifthen}
\providecommand{\eptcs}{{\sl Electronic Proceedings in Theoretical Computer Science}}
\providecommand{\opa}{, Open Publishing Association}
\providecommand{\finishreference}[6]{#1 #2#3, pp. #4--#5, \doi{10.4204/EPTCS.#2.#6}}
\providecommand{\thisvolume}[2][\eptcs]{%
 \ifthenelse{\equal{#2}{13}}{\finishreference{#1}{229}{\opa}{149}{177}{12}}{%
 \ifthenelse{\equal{#2}{1}}{\finishreference{#1}{229}{\opa}{112}{132}{10}}{%
 this volume of #1\opa}}}

